Conformal Semantic Image Segmentation: Post-hoc Quantification of Predictive Uncertainty

We propose a post-hoc, computationally lightweight method to quantify predictive uncertainty in semantic image segmentation. Our approach uses conformal prediction to generate statistically valid prediction sets that are guaranteed to include the ground-truth segmentation mask at a predefined confidence level. We introduce a novel visualization technique of conformalized predictions based on heatmaps, and provide metrics to assess their empirical validity. We demonstrate the effectiveness of our approach on well-known benchmark datasets and image segmentation prediction models, and conclude with practical insights.

==> preamble.tex <==
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
% 

%% === OUR shortcuts ===
%% --- Math, theorem, algorithms editing
\usepackage{bm} %% for fancy math fonts and stuff
\usepackage{bbm} %% for indicator function
\usepackage[ruled,linesnumbered]{algorithm2e}

% === Theorems, etc. ==
\usepackage{amsthm}
\theoremstyle{plain}
% 
\newtheorem{lemma}{Lemma}%[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}%[section]
\newtheorem{corollary}{Corollary}[subsection]
\newtheorem{fact}{Fact}%[section]
\theoremstyle{remark}
\newtheorem*{remark}{Remark}

\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{hypothesis}{Hypothesis}


%% --- Doc editing: style, tables, figures
\RequirePackage[nolist,nohyperlinks]{acronym}
\usepackage{multirow}
\usepackage{subcaption}

%% placeholder for images, among other things
% \usepackage{duckuments}

%% (2) Commands, macros, shortcuts
%% project's github:
\newcommand{\repo}{\url{https://github.com/deel-ai-papers/conformal-segmentation}\xspace}

%%
% \newcommand{\cit}{\textbf{[CIT. NEEDED]}\xspace}

%% === DECLARE Acronyms to be used in the report ===
\begin{acronym}
\acro{UQ}{{Uncertainty Quantification}}
\acro{CP}{{Conformal Prediction}}
\acro{CRC}{{Conformalized Risk Control}}
\acro{ML}{{Machine Learning}}
\acro{DL}{{Deep Learning}}
\acro{UQ}{{Uncertainty Quantification}}
\acro{LAC}{{Least Ambiguous Set-Valued Classifiers}}
\acro{SIS}{{Semantic Image Segmentation}}
\acro{APS}{{Adaptive Prediction Sets}}

\end{acronym}

%% declare SHORTCUTS to avoid typing \ac{..}
\newcommand{\uq}{\ac{UQ}\xspace}
\newcommand{\cp}{\ac{CP}\xspace}
\newcommand{\crc}{\ac{CRC}\xspace}
\newcommand{\ml}{\ac{ML}\xspace}
\newcommand{\dl}{\ac{DL}\xspace}
\newcommand{\seg}{segmentation\xspace}
\newcommand{\vco}{\emph{varisco}\xspace}
\newcommand{\lac}{\ac{LAC}\xspace}
\newcommand{\sis}{\ac{SIS}\xspace}
\newcommand{\aps}{\ac{APS}\xspace}

%% confidence level, risk level
\newcommand{\conf}{$1-\alpha$\xspace}
\newcommand{\al}{$\alpha$\xspace}

\newcommand{\mulmask}{multi-labeled mask\xspace}
\newcommand{\mulmasks}{multi-labeled masks\xspace}

%% === MATH SHORTCUTS ===
\newcommand{\f}{$\widehat{f}$\xspace}
\newcommand{\Yhat}{\widehat{Y}\xspace}
\newcommand{\Chat}{\widehat{C}\xspace}
\newcommand{\lbd}{$\lambda$\xspace}

\newcommand{\lb}{\lambda}
\newcommand{\lbhat}{\hat{\lambda}}
\newcommand{\lbmax}{{\lambda_{\text{max}}}}
\newcommand{\lvec}{\pmb{\lambda}\xspace}
\newcommand{\Lb}{\Lambda}
\newcommand{\Lbhat}{\widehat{\Lambda}}
\newcommand{\fhat}{\widehat{f}}
\newcommand{\Rhat}{\widehat{R}}
\newcommand{\sighat}{\widehat{\sigma}}


\newcommand{\LL}{\mathcal{L}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Dcal}{\mathcal{D}_{\text{cal}}}
\newcommand{\Dval}{\mathcal{D}_{\text{val}}}
\newcommand{\Dtest}{\mathcal{D}_{\text{test}}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\Clb}{\mathcal{C}_{\lambda}}
\newcommand{\Clhat}{\mathcal{C}_{\hat{\lambda}}}
\newcommand{\ncal}{n_{\text{cal}}}
\newcommand{\ntest}{n_{\text{test}}}
\newcommand{\Ih}{\mathcal{I}_{H}}
\newcommand{\Iw}{\mathcal{I}_{W}}
\newcommand{\Ihw}{\mathcal{I}_{HW}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\Caps}{\mathcal{C}^{\text{APS}}}
\newcommand{\Clac}{\mathcal{C}^{\text{LAC}}}
\newcommand{\Iy}{\mathcal{I}_y}

%% === COVERAGE RATIO ===
% \newcommand{\tcov}{\tau_{\text{cov}}}
\newcommand{\tcov}{\tau}



